Morphing Planar Graph Drawings Optimally

We provide an algorithm for computing a planar morph between any two planar straight-line drawings of any $n$-vertex plane graph in $O(n)$ morphing steps, thus improving upon the previously best known $O(n^2)$ upper bound. Further, we prove that our algorithm is optimal, that is, we show that there exist two planar straight-line drawings $\Gamma_s$ and $\Gamma_t$ of an $n$-vertex plane graph $G$ such that any planar morph between $\Gamma_s$ and $\Gamma_t$ requires $\Omega(n)$ morphing steps.

==> commands.tex <==
% % % % % % % epigraph % % % % % % % % %

%\newcommand{\mytextformat}{\itshape\epigraphsize}
%\newenvironment{mytext}{\mytextformat}{}
%\newenvironment{mysource}{\scshape\hfill}{}
%\renewcommand{\textflush}{mytext} 
%\renewcommand{\sourceflush}{mysource}
%
%\let\originalepigraph\epigraph 
%\renewcommand\epigraph[2]%
%   {\setlength{\epigraphwidth}{\widthof{\mytextformat#1}}\originalepigraph{#1}{#2}}

\newcommand{\image}[1]{\includegraphics[scale=0.3]{#1}}
\newcommand{\plot}[1]{\includegraphics[scale=0.55]{#1}}
\newcommand{\remove}[1]{}


%\newtheorem{corollary}{Corollary}
%\newtheorem{definition}{Definition}
%\newtheorem{conjecture}{Conjecture}
\newtheorem{theorem}{Theorem}
%\newtheorem{property}{Property}
\newtheorem{lemma}{Lemma}
%\newtheorem{problem}{Open Problem}
%\newtheorem{observation}{Observation}


\newcommand{\slope}{slope}
\newcommand{\range}{range}
\newcommand{\boom}{boom}
\newcommand{\skel}{skeleton}
\newcommand{\pert}{pertinent}
\newcommand{\diam}{diam}

\newcommand{\host}{x\xspace} %nome del vertice su cui contraiamo
\newcommand{\lhost}{l\xspace} %vicino sinistro del vert su cui contriamo
\newcommand{\rhost}{r\xspace} %vicino destro del vert su cui contriamo
\newcommand{\mhost}{$\host$\xspace}
\newcommand{\mlhost}{$\lhost$\xspace}
\newcommand{\mrhost}{$\rhost$\xspace}
\newcommand{\bm}[1]{\boldmath{$#1$}\xspace}



\newcommand{\morph}[1]{\langle #1 \rangle}
\newcommand{\mmorph}[1]{\ensuremath{\morph{#1}}}
\newcommand{\poly}[1]{\left< #1 \right>}
\newcommand{\mpoly}[1]{\ensuremath{\poly{#1}}}
\newcommand{\seg}[1]{\overline{#1}}
\newcommand{\mseg}[1]{\ensuremath{\seg{#1}}\xspace}
\newcommand{\mcycle}[1]{\ensuremath{#1}}
%\newcommand{\mynote}[1]{\textcolor{red}{\footnote{\color{red}#1}}\xspace}
\newcommand{\mynote}[1]{\textcolor{red}{\footnote{\color{red}#1}} }


\def\dashfill{\cleaders\hbox {-}\hfill}

\newcommand{\todo}[1]{\ \newline \textcolor{red}{TODO:} \textcolor{blue}{#1}\newline}


% % % % % operators % % % % % % % % % % % % % %


% % % % % % % % environments % % % % % % % % %
\newenvironment{proof}
{{\textbf Proof:}}{\hfill$\Box$\par\vspace{1mm}}

\newenvironment{sketch}
{{\em Proof sketch:}}{\hspace*{\fill}$\Box$\par\vspace{2mm}}

% % % % % % % % % % lists % % % % % % % %

%\setdefaultenum{$(i)$}{i.}{A.}{1.}

%\newcommand{\subbottom}[2]{\subfigure[]{#2}}


==> packages.tex <==
\usepackage{varwidth}
%\usepackage{calc}

\usepackage{xcolor}
\usepackage{subfigure}
\usepackage{graphicx}
\usepackage{clrscode}
\usepackage{epsfig}
\usepackage[english]{babel}
\usepackage{graphicx}
\usepackage{amsmath}
%\usepackage[amsmath,thmmarks]{ntheorem}
\usepackage{amssymb}
\usepackage{color}

\usepackage{verbatim}
\usepackage{rotating}
\usepackage{multirow}
\usepackage{makeidx}
\usepackage[pagebackref,hidelinks]{hyperref}
\usepackage[figure]{hypcap}
\usepackage[capitalise]{cleveref}
\usepackage{paralist}
\usepackage{xspace}

\usepackage[plain,ruled]{algorithm}
\usepackage[noend]{algorithmic}
%%\usepackage{algorithmicx}
%\usepackage{algpseudocode}

\usepackage{enumerate}
\usepackage{mdwlist}

%\usepackage{caption}
